Understanding the Role of Large Language Models in Personalizing and Scaffolding Strategies to Combat Academic Procrastination

Traditional interventions for academic procrastination often fail to capture the nuanced, individual-specific factors that underlie them. Large language models (LLMs) hold immense potential for addressing this gap by permitting open-ended inputs, including the ability to customize interventions to individuals' unique needs. However, user expectations and potential limitations of LLMs in this context remain underexplored. To address this, we conducted interviews and focus group discussions with 15 university students and 6 experts, during which a technology probe for generating personalized advice for managing procrastination was presented. Our results highlight the necessity for LLMs to provide structured, deadline-oriented steps and enhanced user support mechanisms. Additionally, our results surface the need for an adaptive approach to questioning based on factors like busyness. These findings offer crucial design implications for the development of LLM-based tools for managing procrastination while cautioning the use of LLMs for therapeutic guidance.

==> CHI_First_Draft/discussion.tex <==
\section{Discussion}

%Our findings contribute to design considerations for tools aimed at managing academic procrastination, particularly in terms of how LLMs can augment existing methodologies. We highlight a few issues \todo{add themes}

In our discussion, we first highlight how our findings answer our research questions, and then we go on to make some design recommendations based on our findings. Finally, we outline the limitations of our study.

\subsection{Key Insights}

\subsubsection{RQ1: Users' Envisioning of LLMs in Managing Academic Procrastination}
In alignment with existing literature on procrastination management and structured goal-setting \cite{pereira2021struggling, grover2020design, brechmann2013remind, das2023focused, hsieh2008using, kovacs2019conservation}, our study reiterates the importance of breaking down larger tasks into more manageable components. LLMs could be particularly well-suited for this, capable of providing both granular, actionable micro-steps for immediate tasks and more abstract guidelines for long-term goals \cite{lin2022applying, mogavi2023exploring}. Participants expected LLMs to be capable of accounting for their unique circumstances and limitations, a feature that can be incorporated by using targeted questions grounded in prior literature \cite{o2018suddenly, d2010problem}. Further customization can be introduced by enhancing instructions with pertinent resources (e.g., links to studies or relevant websites) that can satisfy users' curiosity about the reasoning behind specific steps, thereby allowing them to explore alternative approaches \cite{arakawa2023catalyst, powell2015refined}.

%Participants in our study emphasized the importance of LLMs offering deadline-driven interactions to effectively integrate into their daily routines \cite{pereira2021struggling, grover2020design}. Such a feature would allow individuals to dynamically set task priorities based on the immediacy of deadlines. These findings also contribute to the large body of work on reflection and reminders for managing procrastination \cite{edwards2015examining, martin2015effects, baker2016randomized, humphrey2021exploring, ye2022behavioral, zavaleta2022can}. Our findings indicate that the type of support offered by the LLM could be adaptive, focusing on immediate actions for imminent deadlines while emphasizing alignment with long-term goals when deadlines are distant \cite{oettingen2015rethinking}. These adaptive recommendations could be sent through users' preferred communication medium (e.g., email, text messages, Slack) so that they are integrated within their study or work environment \cite{grover2020design, howe2022design}. Such adaptive support could be informed by previous studies that have personalized reminders and interventions through various communication channels like email and text messages \cite{humphrey2021exploring, ye2022behavioral, zavaleta2022can}.


Participants in our study highlighted the necessity for deadline-oriented interactions facilitated by LLMs as a means of seamlessly integrating into their daily academic activities. This aligns with and extends existing work on the role of reminders and reflection in procrastination management \cite{edwards2015examining, martin2015effects, baker2016randomized, humphrey2021exploring, ye2022behavioral, zavaleta2022can}, allowing for dynamic task prioritization based on the imminence of deadlines. Our findings indicate that the supportive scaffolding provided by the LLM-based tool could adapt based on the time-sensitivity of these deadlines: offering immediate, actionable recommendations for imminent tasks and aligning efforts with broader goals when deadlines are not immediate. These personalized and adaptive prompts could be communicated via channels most convenient to the user (e.g., emails, text messages, Slack) \cite{howe2022design, grover2020design}. This flexibility in communication medium can ensure the tools recommendations can be readily accessed and acted upon, making them more likely to be effective in real-world academic settings \cite{bhattacharjee2023investigating}.



Lastly, our findings revealed a demand among participants for collaborative features in LLM-based tools designed to manage academic procrastination \cite{uzun2013reducing, tuasikal2019role, hsueh2020exploring, bhattacharjee2022kind}. Specifically, participants expressed interest in having a mechanism that allows them to see how others have interacted with the system, including the inputs they have provided and the outputs they have received in return. Implementing such collaborative support can aid users in navigating the complexities of interacting with the LLM-based tool and offer them guidelines or best practices through the experiences of others. However, it also reflects the broader psychological need for communal support in combating procrastination \cite{uzun2013reducing, tuasikal2019role, hsueh2020exploring, burgess2019think}. 

%our study underscores the importance of  Additionally, the integration of deadlines into the system emerged as a critical feature \cite{edwards2015examining, martin2015effects, baker2016randomized, humphrey2021exploring, ye2022behavioral, zavaleta2022can}, facilitating the delivery of context-sensitive notifications. 



%\subsection{Collaborative Support}



\subsubsection{RQ2: Potential Limitations and Tensions}
%\todo{one paragraph on design tension}

%\todo{add cite}
%\subsection{Restrictions in Providing Therapeutic Support}
Our study also sheds light on the limitations of LLMs in the realm of procrastination management, particularly concerning emotional and therapeutic support. These findings align with recent skepticism among clinicians regarding the suitability of LLMs for emotional counseling and therapeutic support \cite{kasneci2023chatgpt, jo2023understanding, mogavi2023exploring}. The experts consulted in our study underscored the need for LLM-based tools to acknowledge and validate user emotions without crossing into the territory of clinical or therapeutic advice \cite{jo2023understanding}. Additionally, they expressed concern about the potential for LLM-based tools to foster overdependence among students \cite{kasneci2023chatgpt, jakesch2023co, mogavi2023exploring}. They warned that easy access to a tool that breaks down complex tasks might inhibit the development of independent problem-solving skills. Consequently, they recommended implementing usage limits and encouraging students to seek their own solutions in order to strike a balance between guided assistance and independent thought \cite{thieme2023foundation}.


We also recognize a design tension regarding the extent of guidance users may wish to see when describing their situation. In some instances, users may prefer a set of structured questions to shape their responses, which may be more feasible during idle periods and moments of downtime \cite{poole2013hci, bhattacharjee2023investigating}. Conversely, a single open-ended question could be more suitable when users are initially acquainting themselves with the system or are in the midst of many other activities \cite{kornfield2020energy}. The same contextual variability applies to the level of customization available in the tool, such as setting the tone, directedness, or length of advice \cite{malle2001attention, bandura1994self, gnambs2010color}. While these features may be beneficial, there are moments when the user may not have the bandwidth to engage with such granularity and would prefer the option to bypass these decisions. 

This situation highlights the need for a design that permits flexible engagement, allowing users to maintain a minimal level of interaction with the system even when they are not fully engaged. Studies in educational psychology and social media behavior indicate that different online activities demand various levels of cognitive involvement \cite{bhattacharjee2023investigating, burke2010social, verduyn2021impact, haidet2004controlled}. While active engagement is typically more beneficial for enhancing learning and wellbeing, our findings suggest that there are times when users may be reluctant to invest significant cognitive effort, particularly during periods of low energy or mood. In such instances, allowing access to essential features without requiring full engagement can be crucial for sustaining a basic level of connection to the support system, thereby avoiding user overwhelm \cite{bhattacharjee2023investigating}.


%A baseline level of such passive interaction can make the system more sustainable for users, particularly during busy or stressful periods, as it lessens the requirement for intense, active engagement that could otherwise discourage continued use.

%This observation aligns with the notion that passive engagement at certain times may actually be beneficial \todo{cite}. It supports previous research suggesting that maintaining a baseline level of passive interaction with a system might be more sustainable for users during periods of high activity or stress, rather than consistently requiring active, intense engagement that could potentially deter ongoing use.




\subsection{Design Recommendations}

Drawing from our findings, we put forth a set of design recommendations aimed at enhancing LLM-based tools for tackling academic procrastination.

\subsubsection{Structured Guidance with Adaptive Complexity}
Future designs for LLM-based procrastination management tools should aim to strike a balance between structure and adaptability to effectively cater to diverse user needs \cite{bhattacharjee2023investigating, liffiton2023codehelp, kazemitabaar2023studying, denny2023promptly, leinonen2023using}. One important feature would be a \textit{dynamic structured guidance system}, designed to generate hierarchical task lists dynamically based on user input \cite{o2018suddenly}. This system could integrate a \textit{task decomposer} function that automatically dissects large tasks into manageable micro-tasks with set deadlines, offering a structured approach to task management \cite{lin2022applying, mogavi2023exploring}. To avoid overwhelming users, the dynamic structured guidance system could initially display immediate sub-tasks in a detailed manner while keeping distant ones more abstract. As users complete the immediate tasks, the system could then automatically 'unlock' detailed information for the subsequent, initially abstract tasks. This staged revelation of task details might allow for a manageable workload  \cite{wu2022ai}, making large tasks feel less daunting. For users who desire further context, a recommendation system could suggest supplemental resources — available via a sidebar or dropdown menu — tailored to each task or sub-task \cite{sallis2015ecological}. Furthermore, the user interface could incorporate a toggle that will allow users to manually adjust the level of task detail.  

\subsubsection{Independent Exploration Prompts}
%\todo{cite}
To mitigate the risk of fostering dependency on the tool \cite{kasneci2023chatgpt}, LLM-based tools could include \textit{independent exploration prompts}. These prompts could offer users various options such as ``research further'', ``think critically'', or ``seek peer advice'', thereby encouraging a range of independent problem-solving activities \cite{loksa2016programming, jin2019solvedeep}. Each option could come with a brief description of what the activity entails and why it might be beneficial, providing a nudge without forcing a specific course of action \cite{bhattacharjee2023design}. These prompts could appear at strategic intervals — perhaps after a pre-defined number of completed sub-tasks or upon reaching significant milestones within a project. Additionally, the system could occasionally force users to explore potential strategies on their own before resuming work with the dynamic structured guidance system \cite{cirillo2018pomodoro, kim2016timeaware}. Users could also have the option to schedule these independent exploration prompts at intervals of their choosing, offering customization to better suit individual work habits and needs \cite{bhattacharjee2023design}.

%\subsubsection{Potential Restriction}


\subsubsection{Integration with Users' Routines}
To achieve seamless integration with users' daily routines, future iterations of LLM-based procrastination management tools could incorporate an \textit{adaptive deadline management} feature. This feature would synchronize with commonly used platforms like Google Calendar, Microsoft Teams, and Slack to automatically import scheduled tasks and deadlines \cite{howe2022design, grover2020design, das2023focused}. Based on this imported information and any user-inputted priorities, the tool could then dynamically generate a ranked task list. In addition to the automatic ranking, a \textit{time-effort estimator} could offer users the option to manually adjust rankings by inputting estimated time commitments and perceived task difficulties \cite{agapie2022longitudinal}. Tailored reminders and motivational cues could then be disseminated to users through their chosen platform \cite{bhattacharjee2023investigating, howe2022design}. Furthermore, the customization of these features could be enhanced by integrating mobile phone sensor data to detect users' activity levels and sleep patterns \cite{ravichandran2017making, daskalova2020sleepbandits}.


%Further integration with user activity level from mobile phone sensor data could also detect periods of inactivity or recognizing gaps between scheduled classes and meetings from calendar schedules. This feature would strategically send productivity prompts or task reminders, ensuring that the tool adapts to the users' real-world contexts while minimizing disruptions.

\subsubsection{Boundaries in Addressing User Emotions}

To guarantee clarity and foster responsible usage, future LLM-based tools for procrastination management should prominently display a detailed disclaimer on the landing page \cite{bhattacharjee2023investigating, bhattacharjee2022kind} that is readily accessible elsewhere within the interface. This disclaimer should explicitly enumerate the tool's capabilities and intended usage while making it clear that it is not capable of providing clinical psychological or emotional support \cite{korngiebel2021considering, ghassemi2021false}. 
% To emphasize this point, the text should include phrases like, ``This tool is not a replacement for professional mental health services or therapeutic intervention.'' 
For users who might require specialized emotional or psychological assistance, the system should also provide a place where users can access a vetted list of well-established resources for mental health support: vetted informational website, helpline numbers, links to accredited mental health service providers, etc. \cite{bhattacharjee2023investigating, bhattacharjee2022kind}.
% dedicated section or button labeled ``Mental Health Resources'' or ``Get Professional Help'', which upon clicking, unfolds to show a list of vetted resources, helpline numbers, and links to accredited mental health service providers \cite{bhattacharjee2023investigating, bhattacharjee2022kind}. 
These cautionary steps can ensure that users are not only informed about what the tool can and cannot do but also have immediate access to more appropriate resources when needed.

%Our findings underscore the imperative to delineate clearly the clinical boundaries of LLM-based tools designed for managing procrastination. 



\subsubsection{Collaborative Support in Using LLM-based Tools}
%https://arxiv.org/pdf/2307.16364.pdf

To provide effective support on the use of LLM-based tools for procrastination management, future systems should emphasize shared experiences and refined feedback mechanisms \cite{bhattacharjee2022kind, burgess2019think, uzun2013reducing, tuasikal2019role, hsueh2020exploring}. To this end, a shared prompt library could be introduced where users can view and contribute diverse examples of effective prompts and corresponding LLM responses. This communal feature would not only allow users to understand the scope of queries they can make but also enable them to learn from one another's experiences \cite{bhattacharjee2022kind}. In terms of feedback, a multi-metric rating system could be implemented \cite{weber2021step} where users could rate the utility, relevance, and clarity of the advice provided by the LLM-based tool along a scale. These ratings could be aggregated and displayed alongside each example in the shared prompt library, serving as additional data for users to gauge the effectiveness of different types of prompts and responses. However, user contributions to this shared resource would need to be thoroughly de-identified to address privacy concerns \cite{thieme2023foundation}.

\subsection{Limitations}

In acknowledging the limitations of our research, we first note that our participant group was composed of individuals residing in North America at the time of the study. Although this cohort included people from various racial groups, the geographical and cultural context in which they live may have influenced their perspectives on the use of LLM-based tools for managing procrastination. Thus, engaging with a different population might reveal unique challenges, preferences, or expectations regarding the use of such tools.

%\todo{Furthermore, we did not do a longitudinal study. While the decision to not deploy the LLM-based tool in real-world scenarios without researcher oversight was made with ethical and risk considerations in mind, this methodological choice may limit our ability to understand the long-term implications and real-world effectiveness of LLM-based tools for procrastination management.}
%There's a lot of value in doing design probe. It also avoids deploying something unvalidated
%we did not do this because ethical reasons. academic, emotional
%Nevertheless, there is still value in doing long term study

Additionally, we designed a technology probe to explore user expectations regarding LLM-based tools for managing academic procrastination. To mitigate academic and emotional risks that could arise from deploying an unvalidated tool, we chose not to conduct a longitudinal study without researcher oversight. Nevertheless, we recognize the potential benefits of long-term studies for a more comprehensive understanding of the real-world effectiveness and long-term implications of LLM-based tools in this context.


==> CHI_First_Draft/findings.tex <==
\section{Findings}
\label{sec: findings}
%\todo{add feedback on the system}
In the following section, we delineate various themes that emerge concerning the ways in which users perceive the utility of LLM-based tools for managing academic procrastination. Additionally, we discuss how expert opinions either corroborate or diverge from these user perspectives.

\subsection{Aspirations for Structured Action Steps}

Participants generally appreciated the flexibility offered by the tool (e.g., the ability to select preferred tone or directedness) for message customization. 
%They found the ability to select preferred tone, directedness, word count, and need for instructions in generating personalized advice useful.
They noted that customization not only enhanced the utility of the tool but also gave them a greater sense of control over their interaction. P1 commented:

\italquote{I think the tone and the length I’d love to play around with, I’m trying to imagine myself as a user. ChatGPT has a tendency to maintain the same tone in all of its messages. I don't think I'm going to the effort of putting this information there. But here people can just directly choose what they want to click in to use.}


Participants also raised potential ideas for additional customization features. For example, some vouched for the ability to switch between action-oriented and suggestive tones, and others suggested the ability to enhance instructions with pertinent resources (e.g., links to studies or relevant websites).  P12 stated that sometimes users may express a desire to understand the reasoning behind a step or to explore alternative approaches, so making such resources available could satiate this curiosity and augment user involvement. However, despite these design opportunities identified by participants, some of them also expressed the concern that an excessive number of options might be overwhelming. To address this, P2 suggested a two-tiered approach: presenting basic customization features on the main page and more advanced options on a separate page.
%While some participants were in favor of adding more customization features, such as selecting between action-oriented and suggestive tones, there was also concern that an excessive number of options might be overwhelming. To address this, P2 suggested a two-tiered approach: presenting basic customization features on the main page and more advanced options on a separate, advanced manipulation page.

Extending this need for customization, participants in our study wished to receive structured guidance from the system to carry out their tasks. Many of them emphasized the challenges they face with unstructured or expansive tasks. The widespread view was that tasks appear more manageable when presented in a clear, step-by-step sequence. 
P8 drew upon a cooking analogy, referencing their preference for following a recipe versus freestyle cooking without any guidance. Beyond ease of use, participants also identified psychological benefits to seeing a concrete action plan. For instance, P2 noted how users could feel fulfillment upon completing individual steps for larger tasks.
% They indicated a preference for more direct, solution-oriented approaches that addressed their specific challenges.
% As P1 suggested:
% \italquote{Maybe give me a really rough plan. And you say like, I should start from what thing and then go towards saying like that.}

Expert insights also underscored the value of offering users assistance in breaking down larger tasks. E1, however, cautioned that while a comprehensive plan can be constructive, there is a risk of overwhelming students. Their recommendation was to detail the imminent steps while providing a broader outline for later tasks. As users navigate through the initial steps, future steps and details can be introduced.
E3 and E6 also raised concerns about fostering over-reliance on the tool. E3 expressed:

\italquote{While structured guidance is valuable, we must ensure students retain their ability for independent thought and action. The danger lies in spoon-feeding them precise answers or solutions. It's crucial for students to develop their own thinking and information-gathering skills. Relying too heavily on a step-by-step model, especially one presented by an LLM, might foster a false sense of accomplishment. Students might follow every instruction and still wonder why their outcomes don't match their expectations.}


%This sense of progressive achievement, as some suggested, has the potential to act as a powerful motivator, spurring them on to the next stages of a task.
In summary, while structured guidance was seen as vital for task management, experts recommended a balance should be struck to ensure learners' independence and critical thinking remain intact.

\subsection{Deadline-Driven Interactions}

Participants appreciated the tool's ability to allow them to draft future emails to themselves. This feature was seen as especially beneficial for managing important deadlines. For instance, P10 indicated they would leverage this capability as a way to document their goals, with the periodic emails serving as reminders to review and refocus on these objectives. P2 and P4 further elaborated that the act of drafting these emails would also assist them in gaining better clarity regarding their goals and plans.

For better management of deadlines, however, several participants expressed an interest in integrating a tool like ours into their daily workflow for on-the-spot, personalized advice and actionable plans. Participants like P2 and P3 suggested integrations with platforms they already use for professional purposes, such as Google Calendar, Microsoft Teams, and Slack. In this context, a recurrent suggestion was the addition of a feature allowing participants to specify task deadlines. They believed that by doing so, the tool would be better positioned to deliver timely and pertinent recommendations. P2 shared an illustrative perspective:

\italquote{I have a friend who will be like, `Yeah, you have this coming up, you have that coming up. So you better do this first and do that first and prioritize this because this is more work than others.' So the AI can somewhat do something similar where you can be like, `You have this coming up. I think you should prioritize this.' It's not like it is telling me to do it. \dots It's just that, like a gentle reminder or something of that fashion.}

Some participants offered thoughts regarding the optimal frequency and timing of reminders from the tool. For instance, P6 emphasized the importance of receiving motivational cues significantly ahead of an impending deadline to prevent last-minute rushes. They went on to suggest incorporating features that allow users to set task priorities and provide estimates for completion times, tailoring the tool's reminders to their individual needs.


Experts largely agreed with the participants but emphasized the diverse motivational needs people require at different times. E2 suggested multiple strategies to this end: for those who feel regret reflecting on past procrastination, a message like ``The past is in the past, focus on today''; for specific barriers, a response inspired by WOOP (wish, outcome, obstacle, plan) goal-setting model \cite{oettingen2015rethinking}; and for a lack of perceived purpose, affirmations connecting tasks to future goals or values. Furthermore, E1 posited that presenting an array of motivational prompts could enable users to select the one that resonates most with them.


%They mentioned situations like a week before important course deadlines, when early prompts could serve to initiate action, especially during moments of inertia. In contrast, they also highlighted the value of last-minute boosts of encouragement to drive completion. As conveyed by their comments, the tool's timing could be critical, offering motivation to start a task at a reasonable time before the deadline.


\subsection{Guided Versus Unguided Questions}
In our prototype, participants had the flexibility to elaborate on their situations to whatever extent they desired. Participants embraced this feature as an opportunity for them to mold canned messages to fit their unique context.
However, opinions varied when discussing the nature and quantity of questions the tool used to probe users for more information. Some participants advocated for a guided approach featuring a sequence of open-ended questions, believing it would help frame their responses more effectively. P7 illustrated this preference by stating, 

\italquote{The first problem is `What is something you are putting off for today?' And then you would write, `I'm putting off x and y'. And then after you type and press [the continue button], it might prompt you to say, `How has that made you feel?' And then it might prompt you to say, `What made me feel this way?'.}

%Despite this preference, participants recognized that spending time writing messages about their situation could unintentionally serve as another source for procrastination. 
Conversely, other participants were concerned that a sequence of questions could serve as a new avenue for procrastination. P2 emphasized the potential to overwhelm users with numerous prompts, especially during initial interactions with the platform. Additionally, building on past experiences with self-management tools, Participant P4 noted that a barrage of questions in the midst of a busy schedule could also heighten stress levels. In scenarios like these, they predicted that users would prefer to receive personalized guidance that is both immediate and easy to access, without the need to navigate through a multitude of questions.
%\todo{individual preferences}

To mitigate these concerns, E1, E3, and E6 suggested the inclusion of adaptive contextual factors to adjust both the quantity and type of questions posed to the user. They recommended employing contextual variables like the time of day, day of the week, and the user's schedule to fine-tune how the LLM elicits more information about the user's situation. While these experts generally supported providing longer interactions informed by psychological literature \cite{schouwenburg2004perspectives, pychyl2013solving}, they also recognized that users should have the option for shorter interactions when experiencing higher levels of activity or stress.

%As a solution, P2 suggested a system where users could choose between more structured, guided questions and more open-ended, unguided ones. They envisioned an interface featuring two distinct buttons, each leading to different levels of guidance in the questions. 

%Expert feedback harmonized with these participant perspectives. E1, while advocating for guided interactions informed by psychological literature, also emphasized the value in letting users opt for shorter interactions, particularly during times of heightened activity or stress.


\subsection{Concerns and Boundaries in Providing Emotional Support}

The recognition and acknowledgment of user emotions emerged as a significant theme, with diverse opinions shared by both participants and experts. They recognized that discussions of procrastination could often lead to revelations about mental states, including symptoms of anxiety and depression. In such cases, some participants expressed the need for emotional support. P4 said:

\italquote{Assuming I already signed up for it, then I might like more emotional support. Like actual links [saying] `Here are resources that you can use'. Maybe there will be options [for showing] pep talks or something like that.}

\noindent
Participants like P7 felt that the tool could be proactive in inquiring users about their emotions and the possible culprits behind negative feelings. P11 went further, expressing an interest in having access to resources for managing more serious and vulnerable issues such as depression.

Nevertheless, experts advised caution regarding the prospect of LLMs taking on roles akin to therapists for providing support in the management of emotions. Their concern stemmed from the possibility that these models could dispense advice that, while perhaps appealing to users, may lack clinical validity. Instead, experts like E1, E4, and E5 emphasized that the tools should only simply recognize users' emotions while clearly communicating their limitations in providing therapeutic support. E3 said:

\italquote{First, acknowledge that the individual is struggling. You know, thank them for the description kind of thing. \ldots Just say this, `This kind of falls out of the scope of what I am able to assist you with'. }

\noindent
E5 elaborated on the need for transparency regarding the tool's limitations, emphasizing that users should be clearly informed from the outset about the tool's capabilities and constraints. This includes an explicit declaration at the introduction page outlining the tool's capacities and the message that any unintentional suggestion regarding emotion management should not be acted upon by users. They further stated that the system should contain contact information for university support services or crisis management centers for further assistance and support.


\subsection{Providing Support on the Use of LLM-based Tools}
Although LLMs are meant to be conversational and intuitive, participants in our study still desired guidance on how to best phrase their responses to get the tool to behave as they anticipated. Some felt that video tutorials and demonstrations might be useful, but there were stronger calls for concrete examples of inputs and outputs. P6 noted that the example prompts in Figure \ref{fig: prompt} helped them learn about the kinds of requests they could make and showed the range of possible outputs they could expect.
%P6 elaborated on this, suggesting that the examples should be diverse in content to illustrate the range of variations that can occur. 
Extending on this idea further, participants proposed the idea of adding a collaborative element so that users could help one another optimally use the tool. P2 expanded on this concept by saying:

\italquote{Maybe share with me what other people are saying as well. So yeah, make it more like a social thing. I would also want to see what other people are asking for in their messages.}

Participants also expressed an interest in providing feedback on the advice generated by the tool so that it would work better for them in the future. Again, they were unsure about how this could be accomplished, so they sought instructions and concrete examples that could assist them in this aspect as well. P2 and P9 went on to suggest that such tools should offer users ways of providing feedback beyond inputs to the LLM. For instance, they envisioned a star-rating system that allows users to evaluate tailored advice on perceived qualities such as relevance, applicability, and level of detail.

Experts concurred with the participants' suggestions, adding an extra layer of caution. E5 stressed that tools need to explicitly distinguish the contexts in which they can be helpful from those in which they cannot. Accordingly, the examples provided to users should be designed to make this distinction abundantly clear so that users are fully aware of the tool's capabilities and limitations.

==> Prototype/discussion.tex <==
\section{Discussion}

%Our findings contribute to design considerations for tools aimed at managing academic procrastination, particularly in terms of how LLMs can augment existing methodologies. We highlight a few issues \todo{add themes}

In our discussion, we first highlight how our findings answer our research questions, and then we go on to make some design recommendations based on our findings. Finally, we outline the limitations of our study.

\subsection{Key Insights}

\subsubsection{RQ1: Users' Envisioning of LLMs in Managing Academic Procrastination}
In alignment with existing literature on procrastination management and structured goal-setting \cite{pereira2021struggling, grover2020design, brechmann2013remind, das2023focused, hsieh2008using, kovacs2019conservation}, our study reiterates the importance of breaking down larger tasks into more manageable components. LLMs could be particularly well-suited for this, capable of providing both granular, actionable micro-steps for immediate tasks and more abstract guidelines for long-term goals \cite{lin2022applying, mogavi2023exploring}. Participants expected LLMs to be capable of accounting for their unique circumstances and limitations, a feature that can be incorporated by using targeted questions grounded in prior literature \cite{o2018suddenly, d2010problem}. Further customization can be introduced by enhancing instructions with pertinent resources (e.g., links to studies or relevant websites) that can satisfy users' curiosity about the reasoning behind specific steps, thereby allowing them to explore alternative approaches \cite{arakawa2023catalyst, powell2015refined}.

%Participants in our study emphasized the importance of LLMs offering deadline-driven interactions to effectively integrate into their daily routines \cite{pereira2021struggling, grover2020design}. Such a feature would allow individuals to dynamically set task priorities based on the immediacy of deadlines. These findings also contribute to the large body of work on reflection and reminders for managing procrastination \cite{edwards2015examining, martin2015effects, baker2016randomized, humphrey2021exploring, ye2022behavioral, zavaleta2022can}. Our findings indicate that the type of support offered by the LLM could be adaptive, focusing on immediate actions for imminent deadlines while emphasizing alignment with long-term goals when deadlines are distant \cite{oettingen2015rethinking}. These adaptive recommendations could be sent through users' preferred communication medium (e.g., email, text messages, Slack) so that they are integrated within their study or work environment \cite{grover2020design, howe2022design}. Such adaptive support could be informed by previous studies that have personalized reminders and interventions through various communication channels like email and text messages \cite{humphrey2021exploring, ye2022behavioral, zavaleta2022can}.


Participants in our study highlighted the necessity for deadline-oriented interactions facilitated by LLMs as a means of seamlessly integrating into their daily academic activities. This aligns with and extends existing work on the role of reminders and reflection in procrastination management \cite{edwards2015examining, martin2015effects, baker2016randomized, humphrey2021exploring, ye2022behavioral, zavaleta2022can}, allowing for dynamic task prioritization based on the imminence of deadlines. Our findings indicate that the supportive scaffolding provided by the LLM-based tool could adapt based on the time-sensitivity of these deadlines: offering immediate, actionable recommendations for imminent tasks and aligning efforts with broader goals when deadlines are not immediate. These personalized and adaptive prompts could be communicated via channels most convenient to the user (e.g., emails, text messages, Slack) \cite{howe2022design, grover2020design}. This flexibility in communication medium can ensure the tools recommendations can be readily accessed and acted upon, making them more likely to be effective in real-world academic settings \cite{bhattacharjee2023investigating}.



Lastly, our findings revealed a demand among participants for collaborative features in LLM-based tools designed to manage academic procrastination \cite{uzun2013reducing, tuasikal2019role, hsueh2020exploring, bhattacharjee2022kind}. Specifically, participants expressed interest in having a mechanism that allows them to see how others have interacted with the system, including the inputs they have provided and the outputs they have received in return. Implementing such collaborative support can aid users in navigating the complexities of interacting with the LLM-based tool and offer them guidelines or best practices through the experiences of others. However, it also reflects the broader psychological need for communal support in combating procrastination \cite{uzun2013reducing, tuasikal2019role, hsueh2020exploring, burgess2019think}. 

%our study underscores the importance of  Additionally, the integration of deadlines into the system emerged as a critical feature \cite{edwards2015examining, martin2015effects, baker2016randomized, humphrey2021exploring, ye2022behavioral, zavaleta2022can}, facilitating the delivery of context-sensitive notifications. 



%\subsection{Collaborative Support}



\subsubsection{RQ2: Potential Limitations and Tensions}
%\todo{one paragraph on design tension}

%\todo{add cite}
%\subsection{Restrictions in Providing Therapeutic Support}
Our study also sheds light on the limitations of LLMs in the realm of procrastination management, particularly concerning emotional and therapeutic support. These findings align with recent skepticism among clinicians regarding the suitability of LLMs for emotional counseling and therapeutic support \cite{kasneci2023chatgpt, jo2023understanding, mogavi2023exploring}. The experts consulted in our study underscored the need for LLM-based tools to acknowledge and validate user emotions without crossing into the territory of clinical or therapeutic advice \cite{jo2023understanding}. Additionally, they expressed concern about the potential for LLM-based tools to foster overdependence among students \cite{kasneci2023chatgpt, jakesch2023co, mogavi2023exploring}. They warned that easy access to a tool that breaks down complex tasks might inhibit the development of independent problem-solving skills. Consequently, they recommended implementing usage limits and encouraging students to seek their own solutions in order to strike a balance between guided assistance and independent thought \cite{thieme2023foundation}.


We also recognize a design tension regarding the extent of guidance users may wish to see when describing their situation. In some instances, users may prefer a set of structured questions to shape their responses, which may be more feasible during idle periods and moments of downtime \cite{poole2013hci, bhattacharjee2023investigating}. Conversely, a single open-ended question could be more suitable when users are initially acquainting themselves with the system or are in the midst of many other activities \cite{kornfield2020energy}. The same contextual variability applies to the level of customization available in the tool, such as setting the tone, directedness, or length of advice \cite{malle2001attention, bandura1994self, gnambs2010color}. While these features may be beneficial, there are moments when the user may not have the bandwidth to engage with such granularity and would prefer the option to bypass these decisions. 

This situation highlights the need for a design that permits flexible engagement, allowing users to maintain a minimal level of interaction with the system even when they are not fully engaged. Studies in educational psychology and social media behavior indicate that different online activities demand various levels of cognitive involvement \cite{bhattacharjee2023investigating, burke2010social, verduyn2021impact, haidet2004controlled}. While active engagement is typically more beneficial for enhancing learning and wellbeing, our findings suggest that there are times when users may be reluctant to invest significant cognitive effort, particularly during periods of low energy or mood. In such instances, allowing access to essential features without requiring full engagement can be crucial for sustaining a basic level of connection to the support system, thereby avoiding user overwhelm \cite{bhattacharjee2023investigating}.


%A baseline level of such passive interaction can make the system more sustainable for users, particularly during busy or stressful periods, as it lessens the requirement for intense, active engagement that could otherwise discourage continued use.

%This observation aligns with the notion that passive engagement at certain times may actually be beneficial \todo{cite}. It supports previous research suggesting that maintaining a baseline level of passive interaction with a system might be more sustainable for users during periods of high activity or stress, rather than consistently requiring active, intense engagement that could potentially deter ongoing use.




\subsection{Design Recommendations}

Drawing from our findings, we put forth a set of design recommendations aimed at enhancing LLM-based tools for tackling academic procrastination.

%\subsubsection{Structured Guidance with Adaptive Complexity}
%Furthermore, the user interface could incorporate a toggle that will allow users to manually adjust the level of task detail.  

\subsubsection{Independent Exploration Prompts}
%\todo{cite}
To mitigate the risk of fostering dependency on the tool \cite{kasneci2023chatgpt}, LLM-based tools could include \textit{independent exploration prompts}. These prompts could offer users various options such as ``research further'', ``think critically'', or ``seek peer advice'', thereby encouraging a range of independent problem-solving activities \cite{loksa2016programming, jin2019solvedeep}. Each option could come with a brief description of what the activity entails and why it might be beneficial, providing a nudge without forcing a specific course of action \cite{bhattacharjee2023design}. These prompts could appear at strategic intervals — perhaps after a pre-defined number of completed sub-tasks or upon reaching significant milestones within a project. Additionally, the system could occasionally force users to explore potential strategies on their own before resuming work with the dynamic structured guidance system \cite{cirillo2018pomodoro, kim2016timeaware}. Users could also have the option to schedule these independent exploration prompts at intervals of their choosing, offering customization to better suit individual work habits and needs \cite{bhattacharjee2023design}.

%\subsubsection{Potential Restriction}


%\subsubsection{Integration with Users' Routines}


%Further integration with user activity level from mobile phone sensor data could also detect periods of inactivity or recognizing gaps between scheduled classes and meetings from calendar schedules. This feature would strategically send productivity prompts or task reminders, ensuring that the tool adapts to the users' real-world contexts while minimizing disruptions.

%\subsubsection{Boundaries in Addressing User Emotions}



%Our findings underscore the imperative to delineate clearly the clinical boundaries of LLM-based tools designed for managing procrastination. 



%\subsubsection{Collaborative Support in Using LLM-based Tools}
%https://arxiv.org/pdf/2307.16364.pdf



\subsection{Limitations}

In acknowledging the limitations of our research, we first note that our participant group was composed of individuals residing in North America at the time of the study. Although this cohort included people from various racial groups, the geographical and cultural context in which they live may have influenced their perspectives on the use of LLM-based tools for managing procrastination. Thus, engaging with a different population might reveal unique challenges, preferences, or expectations regarding the use of such tools.

%\todo{Furthermore, we did not do a longitudinal study. While the decision to not deploy the LLM-based tool in real-world scenarios without researcher oversight was made with ethical and risk considerations in mind, this methodological choice may limit our ability to understand the long-term implications and real-world effectiveness of LLM-based tools for procrastination management.}
%There's a lot of value in doing design probe. It also avoids deploying something unvalidated
%we did not do this because ethical reasons. academic, emotional
%Nevertheless, there is still value in doing long term study

Additionally, we designed a technology probe to explore user expectations regarding LLM-based tools for managing academic procrastination. To mitigate academic and emotional risks that could arise from deploying an unvalidated tool, we chose not to conduct a longitudinal study without researcher oversight. Nevertheless, we recognize the potential benefits of long-term studies for a more comprehensive understanding of the real-world effectiveness and long-term implications of LLM-based tools in this context.


==> Prototype/findings.tex <==
\section{Findings}
\label{sec: findings}
%\todo{add feedback on the system}
In the following section, we delineate various themes that emerge concerning the ways in which users perceive the utility of LLM-based tools for managing academic procrastination. Additionally, we discuss how expert opinions either corroborate or diverge from these user perspectives.

\subsection{Aspirations for Structured Action Steps}

In our prototype, participants had the flexibility to elaborate on their situations to whatever extent they desired. Participants embraced this feature as an opportunity for them to mold canned messages to fit their unique context.
They also appreciated the flexibility offered by the tool (e.g., the ability to select preferred tone or directedness) for message customization. 
%They found the ability to select preferred tone, directedness, word count, and need for instructions in generating personalized advice useful.
They noted that customization not only enhanced the utility of the tool but also gave them a greater sense of control over their interaction. %P1 commented:

%\italquote{I think the tone and the length I’d love to play around with, I’m trying to imagine myself as a user. ChatGPT has a tendency to maintain the same tone in all of its messages. I don't think I'm going to the effort of putting this information there. But here people can just directly choose what they want to click in to use.}
However, opinions varied when discussing the nature and quantity of questions the tool used to probe users for more information. Some participants advocated for a guided approach featuring a sequence of open-ended questions, believing it would help frame their responses more effectively. P7 illustrated this preference by stating, 

\italquote{The first problem is `What is something you are putting off for today?' And then you would write, `I'm putting off x and y'. And then after you type and press [the continue button], it might prompt you to say, `How has that made you feel?' And then it might prompt you to say, `What made me feel this way?'.}

Conversely, other participants were concerned that a sequence of questions could serve as a new avenue for procrastination. P2 emphasized the potential to overwhelm users with numerous prompts, especially during initial interactions with the platform. Additionally, building on past experiences with self-management tools, Participant P4 noted that a barrage of questions in the midst of a busy schedule could also heighten stress levels. In scenarios like these, they predicted that users would prefer to receive personalized guidance that is both immediate and easy to access, without the need to navigate through a multitude of questions.
%\todo{individual preferences}

Participants also raised potential ideas for additional customization features. For example, some vouched for the ability to switch between action-oriented and suggestive tones, and others suggested the ability to enhance instructions with pertinent resources (e.g., links to studies or relevant websites).  P12 stated that sometimes users may express a desire to understand the reasoning behind a step or to explore alternative approaches, so making such resources available could satiate this curiosity and augment user involvement. However, despite these design opportunities identified by participants, some of them also expressed the concern that an excessive number of options might be overwhelming. To address this, P2 suggested a two-tiered approach: presenting basic customization features on the main page and more advanced options on a separate page.
%While some participants were in favor of adding more customization features, such as selecting between action-oriented and suggestive tones, there was also concern that an excessive number of options might be overwhelming. To address this, P2 suggested a two-tiered approach: presenting basic customization features on the main page and more advanced options on a separate, advanced manipulation page.

Extending this need for customization, participants in our study wished to receive structured guidance from the system to carry out their tasks. Many of them emphasized the challenges they face with unstructured or expansive tasks. The widespread view was that tasks appear more manageable when presented in a clear, step-by-step sequence. 
P8 drew upon a cooking analogy, referencing their preference for following a recipe versus freestyle cooking without any guidance. Beyond ease of use, participants also identified psychological benefits to seeing a concrete action plan. For instance, P2 noted how users could feel fulfillment upon completing individual steps for larger tasks.
% They indicated a preference for more direct, solution-oriented approaches that addressed their specific challenges.
% As P1 suggested:
% \italquote{Maybe give me a really rough plan. And you say like, I should start from what thing and then go towards saying like that.}

Expert insights also underscored the value of offering users assistance in breaking down larger tasks. E1, however, cautioned that while a comprehensive plan can be constructive, there is a risk of overwhelming students. Their recommendation was to detail the imminent steps while providing a broader outline for later tasks. As users navigate through the initial steps, future steps and details can be introduced.
E3 and E6 also raised concerns about fostering over-reliance on the tool. E3 expressed:

\italquote{While structured guidance is valuable, we must ensure students retain their ability for independent thought and action. The danger lies in spoon-feeding them precise answers or solutions. It's crucial for students to develop their own thinking and information-gathering skills. Relying too heavily on a step-by-step model, especially one presented by an LLM, might foster a false sense of accomplishment. Students might follow every instruction and still wonder why their outcomes don't match their expectations.}


%This sense of progressive achievement, as some suggested, has the potential to act as a powerful motivator, spurring them on to the next stages of a task.
In summary, while structured guidance was seen as vital for task management, experts recommended a balance should be struck to ensure learners' independence and critical thinking remain intact.

\noindent
\textbf{Implications: }\revision{Future designs for LLM-based procrastination management tools should aim to strike a balance between structure and adaptability to effectively cater to diverse user needs \cite{bhattacharjee2023investigating, liffiton2023codehelp, kazemitabaar2023studying, denny2023promptly, leinonen2023using}. One important feature would be a \textit{dynamic structured guidance system}, designed to generate hierarchical task lists dynamically based on user input \cite{o2018suddenly}. This system could integrate a \textit{task decomposer} function that automatically dissects large tasks into manageable micro-tasks with set deadlines, offering a structured approach to task management \cite{lin2022applying, mogavi2023exploring}. To avoid overwhelming users, the dynamic structured guidance system could initially display immediate sub-tasks in a detailed manner while keeping distant ones more abstract. As users complete the immediate tasks, the system could then automatically 'unlock' detailed information for the subsequent, initially abstract tasks. This staged revelation of task details might allow for a manageable workload  \cite{wu2022ai}, making large tasks feel less daunting. For users who desire further context, a recommendation system could suggest supplemental resources — available via a sidebar or dropdown menu — tailored to each task or sub-task \cite{sallis2015ecological}. Furthermore, the user interface could incorporate a toggle that will allow users to manually adjust the level of task detail.}  

%\subsubsection{Independent Exploration Prompts}
%\todo{cite}
\revision{To mitigate the risk of fostering dependency on the tool \cite{kasneci2023chatgpt}, LLM-based tools could include \textit{independent exploration prompts}. These prompts could offer users various options such as ``research further'', ``think critically'', or ``seek peer advice'', thereby encouraging a range of independent problem-solving activities \cite{loksa2016programming, jin2019solvedeep}. Each option could come with a brief description of what the activity entails and why it might be beneficial, providing a nudge without forcing a specific course of action \cite{bhattacharjee2023design}. These prompts could appear at strategic intervals — perhaps after a pre-defined number of completed sub-tasks or upon reaching significant milestones within a project. Additionally, the system could occasionally force users to explore potential strategies on their own before resuming work with the dynamic structured guidance system \cite{cirillo2018pomodoro, kim2016timeaware}. Users could also have the option to schedule these independent exploration prompts at intervals of their choosing, offering customization to better suit individual work habits and needs \cite{bhattacharjee2023design}.}


\subsection{Deadline-Driven Interactions}

Participants appreciated the tool's ability to allow them to draft future emails to themselves. This feature was seen as especially beneficial for managing important deadlines. For instance, P10 indicated they would leverage this capability as a way to document their goals, with the periodic emails serving as reminders to review and refocus on these objectives. P2 and P4 further elaborated that the act of drafting these emails would also assist them in gaining better clarity regarding their goals and plans.

For better management of deadlines, however, several participants expressed an interest in integrating a tool like ours into their daily workflow for on-the-spot, personalized advice and actionable plans. Participants like P2 and P3 suggested integrations with platforms they already use for professional purposes, such as Google Calendar, Microsoft Teams, and Slack. In this context, a recurrent suggestion was the addition of a feature allowing participants to specify task deadlines. They believed that by doing so, the tool would be better positioned to deliver timely and pertinent recommendations. P2 shared an illustrative perspective:

\italquote{I have a friend who will be like, `Yeah, you have this coming up, you have that coming up. So you better do this first and do that first and prioritize this because this is more work than others.' So the AI can somewhat do something similar where you can be like, `You have this coming up. I think you should prioritize this.' It's not like it is telling me to do it. \dots It's just that, like a gentle reminder or something of that fashion.}

Some participants offered thoughts regarding the optimal frequency and timing of reminders from the tool. For instance, P6 emphasized the importance of receiving motivational cues significantly ahead of an impending deadline to prevent last-minute rushes. They went on to suggest incorporating features that allow users to set task priorities and provide estimates for completion times, tailoring the tool's reminders to their individual needs.


Experts largely agreed with the participants but emphasized the diverse motivational needs people require at different times. E2 suggested multiple strategies to this end: for those who feel regret reflecting on past procrastination, a message like ``The past is in the past, focus on today''; for specific barriers, a response inspired by WOOP (wish, outcome, obstacle, plan) goal-setting model \cite{oettingen2015rethinking}; and for a lack of perceived purpose, affirmations connecting tasks to future goals or values. Furthermore, E1 posited that presenting an array of motivational prompts could enable users to select the one that resonates most with them. E1, E3, and E6 suggested the inclusion of adaptive contextual factors to adjust both the quantity and type of questions posed to the user. They recommended employing contextual variables like the time of day, day of the week, and the user's schedule to fine-tune how the LLM elicits more information about the user's situation. While these experts generally supported providing longer interactions informed by psychological literature \cite{schouwenburg2004perspectives, pychyl2013solving}, they also recognized that users should have the option for shorter interactions when experiencing higher levels of activity or stress.


%They mentioned situations like a week before important course deadlines, when early prompts could serve to initiate action, especially during moments of inertia. In contrast, they also highlighted the value of last-minute boosts of encouragement to drive completion. As conveyed by their comments, the tool's timing could be critical, offering motivation to start a task at a reasonable time before the deadline.


\noindent
\textbf{Implications:} \revision{To achieve seamless integration with users' daily routines, future iterations of LLM-based procrastination management tools could incorporate an \textit{adaptive deadline management} feature. This feature would synchronize with commonly used platforms like Google Calendar, Microsoft Teams, and Slack to automatically import scheduled tasks and deadlines \cite{howe2022design, grover2020design, das2023focused}. Based on this imported information and any user-inputted priorities, the tool could then dynamically generate a ranked task list. In addition to the automatic ranking, a \textit{time-effort estimator} could offer users the option to manually adjust rankings by inputting estimated time commitments and perceived task difficulties \cite{agapie2022longitudinal}. Tailored reminders and motivational cues could then be disseminated to users through their chosen platform \cite{bhattacharjee2023investigating, howe2022design}. Furthermore, the customization of these features could be enhanced by integrating mobile phone sensor data to detect users' activity levels and sleep patterns \cite{ravichandran2017making, daskalova2020sleepbandits}.}


%\subsection{Guided Versus Unguided Questions}


%Despite this preference, participants recognized that spending time writing messages about their situation could unintentionally serve as another source for procrastination. 

%As a solution, P2 suggested a system where users could choose between more structured, guided questions and more open-ended, unguided ones. They envisioned an interface featuring two distinct buttons, each leading to different levels of guidance in the questions. 

%Expert feedback harmonized with these participant perspectives. E1, while advocating for guided interactions informed by psychological literature, also emphasized the value in letting users opt for shorter interactions, particularly during times of heightened activity or stress.

%\noindent
%\textbf{Implications:} Addressing the balance between guided and unguided questions, LLM-based tools should offer flexible modes of interaction. The \textit{dynamic structured guidance system} could be designed to toggle between more detailed, guided interactions and high-level, unguided explorations based on user preference \cite{o2018suddenly, wu2022ai}. The incorporation of \textit{independent exploration prompts} at strategic intervals can cater to users who prefer a more self-directed approach, allowing them to engage in critical thinking or research activities \cite{kasneci2023chatgpt, loksa2016programming, jin2019solvedeep}. These prompts should be customizable, enabling users to decide how often they receive such guidance, thus aligning with their individual interaction preferences \cite{bhattacharjee2023design, cirillo2018pomodoro, kim2016timeaware}.


\subsection{Concerns and Boundaries in Providing Emotional Support}

The recognition and acknowledgment of user emotions emerged as a significant theme, with diverse opinions shared by both participants and experts. They recognized that discussions of procrastination could often lead to revelations about mental states, including symptoms of anxiety and depression. In such cases, some participants expressed the need for emotional support. P4 said:

\italquote{Assuming I already signed up for it, then I might like more emotional support. Like actual links [saying] `Here are resources that you can use'. Maybe there will be options [for showing] pep talks or something like that.}

\noindent
Participants like P7 felt that the tool could be proactive in inquiring users about their emotions and the possible culprits behind negative feelings. P11 went further, expressing an interest in having access to resources for managing more serious and vulnerable issues such as depression.

Nevertheless, experts advised caution regarding the prospect of LLMs taking on roles akin to therapists for providing support in the management of emotions. Their concern stemmed from the possibility that these models could dispense advice that, while perhaps appealing to users, may lack clinical validity. Instead, experts like E1, E4, and E5 emphasized that the tools should only simply recognize users' emotions while clearly communicating their limitations in providing therapeutic support. E3 said:

\italquote{First, acknowledge that the individual is struggling. You know, thank them for the description kind of thing. \ldots Just say this, `This kind of falls out of the scope of what I am able to assist you with'. }

\noindent
E5 elaborated on the need for transparency regarding the tool's limitations, emphasizing that users should be clearly informed from the outset about the tool's capabilities and constraints. This includes an explicit declaration at the introduction page outlining the tool's capacities and the message that any unintentional suggestion regarding emotion management should not be acted upon by users. They further stated that the system should contain contact information for university support services or crisis management centers for further assistance and support.


\noindent
\textbf{Implications:} \revision{To guarantee clarity and foster responsible usage, future LLM-based tools for procrastination management should prominently display a detailed disclaimer on the landing page \cite{bhattacharjee2023investigating, bhattacharjee2022kind} that is readily accessible elsewhere within the interface. This disclaimer should explicitly enumerate the tool's capabilities and intended usage while making it clear that it is not capable of providing clinical psychological or emotional support \cite{korngiebel2021considering, ghassemi2021false}. 
% To emphasize this point, the text should include phrases like, ``This tool is not a replacement for professional mental health services or therapeutic intervention.'' 
For users who might require specialized emotional or psychological assistance, the system should also provide a place where users can access a vetted list of well-established resources for mental health support: vetted informational website, helpline numbers, links to accredited mental health service providers, etc. \cite{bhattacharjee2023investigating, bhattacharjee2022kind}.
% dedicated section or button labeled ``Mental Health Resources'' or ``Get Professional Help'', which upon clicking, unfolds to show a list of vetted resources, helpline numbers, and links to accredited mental health service providers \cite{bhattacharjee2023investigating, bhattacharjee2022kind}. 
These cautionary steps can ensure that users are not only informed about what the tool can and cannot do but also have immediate access to more appropriate resources when needed.}

%Our findings underscore the imperative to delineate clearly the clinical boundaries of LLM-based tools designed for managing procrastination. 


\subsection{Providing Support on the Use of LLM-based Tools}
Although LLMs are meant to be conversational and intuitive, participants in our study still desired guidance on how to best phrase their responses to get the tool to behave as they anticipated. Some felt that video tutorials and demonstrations might be useful, but there were stronger calls for concrete examples of inputs and outputs. P6 noted that the example prompts in Figure \ref{fig: prompt} helped them learn about the kinds of requests they could make and showed the range of possible outputs they could expect.
%P6 elaborated on this, suggesting that the examples should be diverse in content to illustrate the range of variations that can occur. 
Extending on this idea further, participants proposed the idea of adding a collaborative element so that users could help one another optimally use the tool. P2 expanded on this concept by saying:

\italquote{Maybe share with me what other people are saying as well. So yeah, make it more like a social thing. I would also want to see what other people are asking for in their messages.}

Participants also expressed an interest in providing feedback on the advice generated by the tool so that it would work better for them in the future. Again, they were unsure about how this could be accomplished, so they sought instructions and concrete examples that could assist them in this aspect as well. P2 and P9 went on to suggest that such tools should offer users ways of providing feedback beyond inputs to the LLM. For instance, they envisioned a star-rating system that allows users to evaluate tailored advice on perceived qualities such as relevance, applicability, and level of detail.

Experts concurred with the participants' suggestions, adding an extra layer of caution. E5 stressed that tools need to explicitly distinguish the contexts in which they can be helpful from those in which they cannot. Accordingly, the examples provided to users should be designed to make this distinction abundantly clear so that users are fully aware of the tool's capabilities and limitations.

\noindent
\textbf{Implications:} \revision{To provide effective support on the use of LLM-based tools for procrastination management, future systems should emphasize shared experiences and refined feedback mechanisms \cite{bhattacharjee2022kind, burgess2019think, uzun2013reducing, tuasikal2019role, hsueh2020exploring}. To this end, a shared prompt library could be introduced where users can view and contribute diverse examples of effective prompts and corresponding LLM responses. This communal feature would not only allow users to understand the scope of queries they can make but also enable them to learn from one another's experiences \cite{bhattacharjee2022kind}. In terms of feedback, a multi-metric rating system could be implemented \cite{weber2021step} where users could rate the utility, relevance, and clarity of the advice provided by the LLM-based tool along a scale. These ratings could be aggregated and displayed alongside each example in the shared prompt library, serving as additional data for users to gauge the effectiveness of different types of prompts and responses. However, user contributions to this shared resource would need to be thoroughly de-identified to address privacy concerns \cite{thieme2023foundation}.}


==> draft/design.tex <==

\section{Design of the Prototype}
LLMs are being integrated in a variety of settings in day-to-day tools. However, due to \todo{why did we choose procrastination?}, our research efforts are concentrated on the application of LLMs in a specific yet prevalent and indicative setting -- procrastination management -- leading us to create our own intervention for said purpose. The form of intervention chosen was a web-app named \textit{Self-Generated Personalized Articulations and Reflections Kit}, or SPARK, hosted on the internet publicly. 

The goal of SPARK was to design an interface that guides students in providing details about their habits and challenges to receive personalized advice from LLMs on how to manage their specific situation of procrastination. 

\begin{figure}[h]
\includegraphics[width=11cm]{spark-feature0.png}
\caption{SPARK landing page}
\centering
\end{figure}

After getting the user's name in the landing page (see Fig 1), the user is led to the main features of SPARK.

SPARK has three main features:  1) providing LLM-generated responses to users' self-described struggles with procrastination, and 2) a space for users to write messages about their future self, with LLM-support in imagining their future and editing the message, which ultimately will be sent to the user's provided email at a self-chosen date and time.


\begin{figure}[h]
\includegraphics[width=12cm]{spark-feature1.png}
\caption{Snapshot of feature 1}
\centering
\end{figure}
The first feature is in the form of story writing, where users provide any details they feel necessary about their struggles with procrastination, aimed at provoking personal reflection. After entering their situation, they can play with LLM-prompt options, including:
tone, directness, length of LLM-response, whether or not the response should include instructions to help with their situation, and prompts to generate the response with, shown in Fig 3.

These LLM-prompt options are chosen to give the user the freedom and power to generate a personalised LLM-response based on their preferences in the type of response they would like to receive. 
Tone (Formal, Informal) refers to the overall feeling or attitude conveyed in the message. Different tones will have different effects based on the situation and audience.
Directness (Direct, Indirect) refers to the degree to which the message is explicit and to-the-point. A user would benefit from a more direct response if they would like to receive feedback that is more straightforward, and more elaborate otherwise.
Length (50, 100 or 150 words) of the LLM-response can greatly impact its effectiveness. Providing users with this option can allow the response to deliver the necessary content in a length as concise or comprehensive as the user wishes.
The option to include instructions gives users the choice to receive direct guidance on how to achieve a particular outcome to navigate their self-described struggles. However, it is also a common pattern that some forms of seeking help is ultimately for venting purposes. In those cases, instructions on improving their situation is not necessary -- they just want to be heard and understood.

\begin{figure}[h]
\includegraphics[width=11cm]{spark-feature1-1.png}
\caption{Prompt options to generate LLM-response}
\centering
\end{figure}

Finally, the user is also provided with prompts to generate the LLM-response with. As shown in Fig 3, the selection of prompts provided represent 5 corresponding styles: motivating, inspirational, scientific, concise, and customization (users create their own prompt). After selecting all the LLM-prompt options, the user can finally generate a message tailored to their situation, as demonstrated in Fig 4 (where the first prompt chosen, i.e. "make it in the tone of a coach trying to motivate a person").


\begin{figure}[h]
\includegraphics[width=14cm]{spark-feature1-2.png}
\caption{LLM-response example}
\centering
\end{figure}

After receiving the LLM-response, the user can choose to edit the response (Fig 5 - Left) or make open-ended LLM-requests, such as improving grammar/spelling or changing the tone of the message (Fig 5 - Right).

\begin{figure}%
    \centering
    {{\includegraphics[width=6cm]{spark-feature1-3.png}}}%
    \qquad
    {{\includegraphics[width=5cm]{spark-feature1-4.png} }}%
    \caption{Making more edits or GPT-requests}%

\end{figure}



==> draft/introduction.tex <==
\section{Introduction}

%procrastination is a big problem - 
Procrastination, defined as the intentional delay of tasks despite known negative consequences \todo{cite}, is especially widespread in academic settings. Prior research indicates that at least half of all college students engage in chronic procrastination \cite{steel2007nature}, which can negatively impact their academic performance and overall wellbeing.
To mitigate this, researchers have developed a range of interventions focusing on task completion \todo{cite}, time management \todo{cite}, and motivation \todo{cite}. %For instance, some interventions use the Pomodoro technique for time management \todo{cite}, while some others deploy machine learning for personalized motivational messages \todo{cite}.
%Driven by the negative impact of procrastination, various interventions have been researched to assist students \todo{cite}. These often target specific task completion, time management, or motivation. For example, some tools utilize the Pomodoro technique to structure work time \todo{cite}, while others employ machine learning to tailor motivational messages \todo{cite}.
%This phenomenon can manifest as a disconnection between one's intentions and subsequent actions, where an individual's goals and the required steps to reach those goals are misaligned \todo{cite}. 
%Such behavior frequently leads to delays in completing academic assignments and coursework. Consequently, affected students often underperform relative to their potential, which has adverse implications for their academic success, future career prospects, and overall wellbeing.
%tools do not contextualize recommendations
%Motivated by the detrimental consequences of procrastination, researchers have developed a range of interventions and tools aimed at aiding students \todo{cite}. These solutions often focus on specific task completion \todo{cite}, time management \todo{cite}, and motivational enhancement \todo{cite}. For instance, one such tool may employ a Pomodoro technique to help students break their work into manageable intervals \todo{cite}, while another may utilize machine learning algorithms to personalize motivational messages \todo{cite}. 
However, a common concern is that these tools often dispense advice that is not sufficiently tailored to individual student contexts. As a result, students frequently struggle to understand how to apply a given piece of advice effectively in their own situations. For example, a time-management app that suggests allocating four uninterrupted hours for study might not take into account a student's part-time job or family responsibilities. In such cases, the app's advice, although well-intended, may not be practical for the individual student's real-world constraints. Another example could be a study guide app that proposes a generic study plan for final exams, not considering that some students may need to prioritize certain subjects over others based on their individual strengths and weaknesses. These nuances of an individual's life could  be challenging to capture under simpler algorithms or recommendation systems that often operate on predefined rules.


%examples highlight the limitations of one-size-fits-all approaches and underline the need for more context-sensitive solutions.

%LLMs have the promise to contextualize, but new tool with limitations as well
With the recent emergence of large language models (LLMs), one might hope that providing more context-sensitive suggestions might be possible. LLMs can analyze vast amounts of data to generate more nuanced and personalized responses. This is particularly important when dealing with complex issues like procrastination, which can be influenced by a multitude of factors such as individual psychology, external environment, and specific task requirements. LLMs have the potential to tailor advice or suggestions based on the specific context provided by the user. For example, if a student is procrastinating on a particular type of task, the LLM may be able to offer targeted strategies that address the unique challenges posed by that task. Furthermore, the adaptability and learning capabilities of LLMs could enable them to refine their recommendations over time, learning from user interactions to provide increasingly effective and personalized support. 


%Challenges too
However, there are several challenges to consider. First, these models are often seen as ``black boxes'', making it difficult to tweak their architecture for specific needs. Second, they can perpetuate existing biases or offer advice that is not scientifically valid. This becomes particularly concerning in cases where users may be struggling with mental health symptoms like anxiety or depression; an LLM could inadvertently provide recommendations that lack clinical validity. Lastly, the user experience could be less than intuitive, as these models often require inputs to be formatted in specific ways that may not be easily understood by the average user.

Given the intricacies and limitations of LLMs, our study aims to gain insights into user needs for a procrastination management tool enhanced by LLMs. Our guiding research question refines the focus to: \textit{What key considerations should designers account for when incorporating LLMs into procrastination management tools?}



\textit{To what extent can Large Language Models augment existing strategies for managing academic procrastination?}


\todo{key design elements}


%We are motivated to take a first step toward understanding how to leverage LLMs in helping students manage procrastination

==> draft/michael--notes.tex <==
What design recommendations do stakeholders want to see when using (SPARK) LLM-integrated proc...mngmt...?

Creators/Researchers \& Instructors
\begin{itemize}
    \item What evidence do they have that this works? (WHY should I do it?)
    \item What are the potential downsides to running this in my class/giving this to my students? 
    \begin{itemize}
        \item What assurances can you (creator of SPARK) give us (Instructors) to be able to implement this with MINIMAL harm to our community? 
    \end{itemize}
    \item What can I do to customize the solution for an individual student in my class (e.g., I have thousands of students, how do I reach them uniquely?)?
\end{itemize}

Users (people seeking help a.k.a. students)
\begin{itemize}
    \item Is this tool endorsed by my instructor/institution? 
    \item Who is seeing what I write and can this potentially come back and bite me in the behind (as in.. if I confess to cheating, can they use it against me?)? 
    \item If I really need help... does a human get a message? 
    \begin{itemize}
        \item This is an opportunity to ensure clarity of who is reading the data and what it's being for is transparent. 
    \end{itemize}
    % BACK TO MAIN GOAL!!
    \item What are things I liked about the usability of the system, and what didn't I like? 
    \begin{itemize}
        \item THE WHY? Why do I (student) care about this particular feature --- relate it back to a quote ... which talks about how it made them feel (personal, strategic/operational, etc..). 
        \item WHAT helped with procrastination? -- take a quote or two and analyze it. 
    \end{itemize}
    \item (might not exist in your data) What from this system did students feel like replicated them talking to a real person. (this might be implicity) ... but I think that the conversational aspect is going to be key here... it'll relate back to conversational agents, but also ITSs/ITAs (Intelligent Tutoring Systems/Intelligent Teaching Assistants) --- the link will exist because it's likely personalized advice a TA would give to a student.
    \item USABILITY/FEATURE GUIDE --- the current call in the student community is X, Y, Z,..., where we (researchers) can use this information to develop this. 
\end{itemize}


==> draft/related_work.tex <==
\section{Related Work}

We first delve into existing literature concerning the application of LLMs in academic environments, focusing specifically on their use in personalization and contextual adaptation, their role as a supportive scaffold, and the ethical challenges that arise from their use. Subsequently, we turn our attention to prior interventions aimed at mitigating academic procrastination.


\subsection{Application of LLMs in Academic Settings}
%https://dbuschek.medium.com/uist23-preprint-collection-18a005356aa5

The emergence of LLMs has introduced new possibilities in learning and education. Within academic settings, they can serve multiple roles — from personalizing learning experiences to providing task-oriented support \cite{mogavi2023exploring, tian2023last, arakawa2023catalyst, yuan2022wordcraft, abd2023large}. As a result, researchers have started employing LLM-based tools in different phases of education, including content creation and summarization, student evaluation, collaborative data analysis, and research \cite{dang2023choice, mogavi2023exploring, abd2023large, wang2023next, halaweh2023chatgpt, kumar2023exploring}.

%\todo{divide into subsections}
%\todo{cite}
One of the most salient strengths of LLMs in educational settings is their capacity for personalization and contextual adaptation \cite{wang2023enabling, kumar2023exploring, dang2023choice, kong2023investigating}. For instance, educational platforms equipped with LLMs have been used to analyze the historical data of a student's essay submissions, allowing them to suggest areas of improvement \cite{uchiyama2023large} and to identify recurring grammatical errors or stylistic issues \cite{dang2023choice, moore2023empowering, mogavi2023exploring, williamson2023re}. In programming courses, LLMs can act as adaptable tutors that provide hints or suggest debugging strategies when students encounter errors in their code \cite{liffiton2023codehelp, kazemitabaar2023studying, denny2023promptly, leinonen2023using}. Unlike static FAQs or forums, the generated advice can take into account the specific syntax and logic of the student's work. Furthermore, LLMs have the potential to facilitate personalized learning journeys by recommending courses or materials that correspond with an individual's academic objectives and interests \cite{kasneci2023chatgpt, bhutoria2022personalized, morreel2023aye}. To illustrate, if a student indicates a desire to achieve proficiency in a specific programming language, an LLM could suggest a series of progressively challenging exercises and relevant readings, thereby offering a bespoke pathway toward mastery \cite{mogavi2023exploring}.

%\todo{cite}
Beyond their capacity for personalization, LLMs can excel as supportive scaffolds in academic tasks that require additional guidance or collaborative input \cite{lee2022coauthor, yuan2022wordcraft, arakawa2023catalyst, zhu2022action, kim2022learning, denny2023conversing, imani2023industry}. In writing-intensive courses, LLMs can function as intelligent writing assistants \cite{lee2022coauthor, gmeiner2023dimensions, kim2023towards, wei2022chain}; they can provide more than mere copy-editing, but also real-time support in even enhancing the structure and flow of arguments. They can also assist students in brainstorming ideas, organizing their thoughts, and co-creating outlines for essays or research papers \cite{kasneci2023chatgpt, abd2023large, zhang2023benchmarking, tang2023evaluating, kitamura2023chatgpt}. Additionally, LLMs can be helpful for microlearning experiences, particularly in subjects that involve complex scientific concepts \cite{lin2022applying, mogavi2023exploring}. By breaking down complex ideas into digestible and more comprehensible explanations, they might offer students a way to incrementally strengthen their understanding.

%\todo{cite}
While the promises of LLMs in academic settings are manifold, these benefits come with ethical concerns that cannot be ignored \cite{lund2023chatgpt, thirunavukarasu2023large, jakesch2023co, kasneci2023chatgpt, jo2023understanding, bender2021dangers}. One significant worry is the potentially detrimental impact LLMs can have on critical thinking and problem-solving skills \cite{kasneci2023chatgpt, jakesch2023co}. The ease and immediacy of AI-generated responses may discourage students from delving deeply into subjects, opting instead for quick answers without a solid understanding of underlying principles \cite{mogavi2023exploring, jakesch2023co, milano2023large}. This issue is exacerbated by the possibility that students may rely too heavily on LLMs, diminishing traditional student-teacher interactions that are often essential for learning \cite{milano2023large}. There is also the problem of accuracy \cite{dale2022detecting, pagnoni2021understanding, pavlik2023collaborating}. Students might not question the validity of the information provided by LLMs under the false assumption that any machine-generated information must be correct. This could lead to the unintentional dissemination of false or misleading information \cite{thieme2023foundation, korngiebel2021considering}. Such concerns could be heightened in the specific context of academic procrastination management, where erroneous or contextually inappropriate advice could have detrimental effects \cite{jo2023understanding}.  
These ethical issues bring into focus the need for careful design and implementation strategies when incorporating LLMs into academic environments.


%Research has demonstrated a growing interest in LLMs due to their capabilities to deliver personalized responses, adaptability to the pace and learning style of students, and their high accessibility \cite{mogavi2023exploring, tian2023last, arakawa2023catalyst, yuan2022wordcraft, abd2023large}. 
%Researchers have started employing LLM-based tools in different phases of education, including content creation and summarizing, student evaluation, collaborative data analysis, and research \cite{mogavi2023exploring, abd2023large, wang2023next, halaweh2023chatgpt}. 

%\todo{find more studies from abd2023large}

%In an in-depth qualitative examination of user-generated content from social media platforms, \citet{mogavi2023exploring} investigated the user experience (UX) and opinions of early adopters towards the AI chatbot technology, specifically ChatGPT, across different educational settings. While their study suggests that ChatGPT has the potential to contribute to increasing self-confidence and motivation among learners, it also highlights potential restrictions these systems might impose on the development of students' social and critical thinking skills.

\subsection{Interventions to Manage Procrastination}

\todo{Alex feedback: fix organization of these paragraphs}

Interventions aimed at mitigating procrastination have been varied and multifaceted, reflecting the complex nature of the problem. They can be broadly categorized into three categories \cite{schouwenburg2004perspectives, van2018overcoming}: 
% (1) techniques that enhance self-regulatory skills \cite{posner2000developing}, nurturing positive habits like goal setting, time management, and distraction minimization \cite{steel2007nature, cirillo2018pomodoro, kim2016timeaware}; (2) techniques that bolster self-efficacy \cite{bandura1994self}, targeting the transformation of negative thinking patterns into motivational thoughts \cite{rozental2015internet, toker2015effect}; and (3) techniques that facilitate social support, recognizing the shared struggles among procrastinators in order to foster collective problem-solving and encouragement \cite{uzun2013reducing, tuasikal2019role, hsueh2020exploring}. 
\begin{enumerate}
\item Techniques that enhance self-regulatory skills \cite{posner2000developing}, nurturing positive habits like goal setting, time management, and distraction minimization \cite{steel2007nature, cirillo2018pomodoro, kim2016timeaware}
\item Techniques that bolster self-efficacy \cite{bandura1994self}, targeting the transformation of negative thinking patterns into motivational thoughts \cite{rozental2015internet, toker2015effect} 
\item Techniques that facilitate social support, recognizing the shared struggles among procrastinators in order to foster collective problem-solving and encouragement \cite{uzun2013reducing, tuasikal2019role, hsueh2020exploring}.
\end{enumerate}

\noindent
These traditional approaches aim to bridge the gap between intention and action \cite{sheeran2016intention, gollwitzer2006implementation}, a central challenge in tackling procrastination. They have been crafted to address this issue through diverse methods, including self-help exercises, guided workshops, and therapeutic sessions \cite{pychyl2013solving, van2018overcoming}.  

%\todo{in the CHI community, people did XYZ}

These works have motivated HCI researchers to create several specialized tools to provide support for distinct use cases \cite{inie2021aiki, arakawa2023catalyst, kovacs2019conservation, kim2016timeaware, hsueh2020exploring}. For instance, \citet{inie2021aiki} developed a browser extension that intervenes when users try to access websites that are likely to waste time, offering them microlearning activities and incorporating feedback loops. In a related endeavor, \citet{kim2016timeaware} created a system for self-monitoring productivity. They discovered that users who reflected on periods of distraction were more likely to decrease procrastinatory behavior. More recently, \citet{arakawa2023catalyst} devised a platform that utilizes generative AI models to help individuals resume interrupted tasks by supplying contextual cues, thus facilitating a smoother transition back to the task.

A range of studies have concentrated on assisting individuals in achieving their goals and deadlines by facilitating increased time spent on focused tasks \cite{pereira2021struggling, grover2020design, brechmann2013remind, das2023focused, hsieh2008using, kovacs2019conservation}. For instance, \citet{pereira2021struggling} examined the effectiveness of GanttBot, a Telegram chatbot designed to reduce procrastination in single-student capstone projects. Incorporating various features like alerts, advice, automatic rescheduling, motivational messages, and historical project references, the chatbot was successful in reducing the number of overdue days among students compared to a control group. A chatbot developed by \citet{grover2020design} that allowed information workers to block out time in calendars and reflect on daily mood also saw similar success in helping them spend more time on focused tasks. However, \cite{kovacs2019conservation} caution that while such interventions may effectively reduce procrastination in targeted settings, they could potentially shift procrastinatory behaviors to other areas, emphasizing the need for a holistic approach.

Finally,  a considerable body of research has focused on mitigating procrastination in academic environments through various reflection and reminder mechanisms, such as emails and text messages \cite{edwards2015examining, martin2015effects, baker2016randomized, humphrey2021exploring, ye2022behavioral, zavaleta2022can}. One such study by \citet{edwards2015examining} employed email reminders to update students on their previous homework performance, which led to a significant decline in late submissions and an uptick in early ones. Supporting this finding, \citet{ye2022behavioral} also found that email reminders could have a positive impact on academic grades. However, \citet{humphrey2021exploring} reported that text message reminders could also encourage timely submissions and enhance overall academic performance. Taken together, these studies contribute to an evolving understanding of how to effectively design messages that both motivate students to commence their work early and remind them of impending deadlines.

%\todo{add goalsetting studies}

%These specialized tools add another layer to the broader discussion on how to support individuals in managing procrastination and improving productivity.

A recurring critique of these interventions is their frequent inability to address the complex, individualized factors that contribute to procrastination \cite{kovacs2019conservation, bhattacharjee2023investigating}. Factors such as social circumstances, motivational triggers, or unique lifestyles are often challenging to incorporate into these designs. Addressing such nuanced issues could potentially benefit from the open-ended input capabilities of LLMs. However, there is a notable gap in understanding how users might perceive and interact with these LLM systems, how LLMs could enhance existing interventions, and what challenges and ethical considerations may be associated with their use. Our study aims to delve into these issues.





%While these solutions have shown promise, \citet{kovacs2019conservation} observed that certain interventions might increase focus on primary goals but may negatively impact time allocation in other life aspects.

%\todo{add cite}
%Despite the above advancements, a comprehensive understanding of what users specifically desire from a procrastination management platform remains elusive in the CHI community. Previous psychological studies have highlighted the importance of time management, goal setting, and collaboration in procrastination interventions. However, a recurring user concern is the lack of specificity and context-awareness in these solutions. LLMs present a potentially powerful means of addressing these issues, but they must be meticulously crafted to be effective. These challenges and opportunities drive our inquiry into user expectations and requirements from procrastination management platforms, as well as the limitations and challenges to be aware of.






%Various interventions have been designed to combat procrastination, employing an array of approaches. Traditional strategies have often focused on time management, such as the Eisenhower Matrix for task prioritization \cite{covey1989seven}, or the use of digital reminders and schedules (Steel, 2007). More recently, specialized techniques like the Pomodoro Technique have gained popularity, segmenting work into focused intervals to enhance concentration and reduce burnout (Cirillo, 2007; Ostendorf et al., 2019). Advances in technology have also allowed for the creation of AI-driven adaptive systems that provide dynamic customization based on individual behavior, learning patterns, and performance metrics (Wang et al., 2018; Alhadreti & Mayhew, 2017). Moreover, gamified applications that make task completion competitive and rewarding have found traction (Hamari et al., 2014; Zichermann & Cunningham, 2011).

